ReBound: An Open-Source 3D Bounding Box Annotation Tool for Active Learning

In recent years, supervised learning has become the dominant paradigm for training deep-learning based methods for 3D object detection. Lately, the academic community has studied 3D object detection in the context of autonomous vehicles (AVs) using publicly available datasets such as nuScenes and Argoverse 2.0. However, these datasets may have incomplete annotations, often only labeling a small subset of objects in a scene. Although commercial services exists for 3D bounding box annotation, these are often prohibitively expensive. To address these limitations, we propose ReBound, an open-source 3D visualization and dataset re-annotation tool that works across different datasets. In this paper, we detail the design of our tool and present survey results that highlight the usability of our software. Further, we show that ReBound is effective for exploratory data analysis and can facilitate active-learning. Our code and documentation is available at https://github.com/ajedgley/ReBound

==> backup.tex <==
\section{Related Work}

In this section we present a brief overview of related work on 3D annotation tools and active learning for object detection. 

\textbf{3D Annotation Tools.}
 Modern 3D detectors require diverse, large-scale 3D annotations. A variety of tools have been created to address this challenge \cite{li20_autochallenges}, including labelCloud\cite{sager21_labelcloud}, SAnE\cite{arief20_sane}, LATTE\cite{wang19_latte}, and 3D BAT\cite{zimmer19_bat}. These products provide convenient ways of labeling raw point cloud data, often for the purpose of autonomous driving applications. However, unlike existing tools, ReBound is able to modify existing datasets for evolving use cases. In addition, our tool works by converting the data from dataset-specific data types into a generic data format. It focuses on efficiently allowing users to edit this existing data, either through the modification of offset bounding boxes or the correction of incorrect object labels. The tool also has the ability to create new categories for classification, which allows users to mold the existing data to be more specified. For instance, if a dataset converted into our generic format had a category for miscellaneous objects and a researcher wanted to be able to easily identify traffic cones in the labels, our tool provides the functionality to add this new class and change existing miscellaneous box labels to match it, something that the aforementioned annotation tools do not do as they are limited by stricter lists of classes. Currently, our tool has the functionality to use data from the nuScenes\cite{caesar20_nuscenes}, Waymo Open Dataset\cite{sun20_waymo}, and Argoverse 2.0\cite{wilson21_argo} datasets. Through the conversion of these outside data formats to our generic ReBound form, these datasets can also be used in conjunction to provide a wider range of training and test data for autonomous driving research projects, which is a service that other similar tools do not provide.

\textbf{Active Learning for Object Detection.} 
%Common methods of decision-making in modern autonomous driving research and implementations are State Machine, Decision Tree, Deep Learning, Reinforcement Learning, and Inverse Reinforcement Learning. Each approach has its own pros and cons of use \cite{dingyi18_trends}. 
 Despite substantial progress of active learning for image recognition, active learning  for object detection is limited. Several studies have been done to assess the potential of this active learning in object detection \cite{haussmann20_activeobj, feng19_trainactive, roy18_deepactive}. Uncertainty about semantics and localization.  \cite{MIAOD2021} proposes to select the most informative images for detector training by observing instance-level uncertainty. However, there is potential to use active learning in training for 3D object detection .

 We provide the ability to modify any incorrect bounding boxes and labels, create custom labels to expand the vocabulary, compare and filter both ground truth and prediction annotations, and export annotation modifications. Data filtering
